HyperForce: Hypervisor-enForced Execution of Security-Critical Code

The sustained popularity of the cloud and cloud-related services accelerate the evolution of virtualization-enabling technologies. Modern off-the-shelf computers are already equipped with specialized hardware that enables a hypervisor to manage the simultaneous execution of multiple operating systems. Researchers have proposed security mechanisms that operate within such a hypervisor to protect the \textit{virtualized} operating systems from attacks. These mechanisms improve in security over previous techniques since the defense system is no longer part of an operating system's attack surface. However, due to constant transitions between the hypervisor and the operating systems, these countermeasures typically incur a significant performance overhead. In this paper we present HyperForce, a framework which allows the deployment of security-critical code in a way that significantly outperforms previous \textit{in-hypervisor} systems while maintaining similar guarantees with respect to security and integrity. HyperForce is a hybrid system which combines the performance of an \textit{in-guest} security mechanism with the security of in-hypervisor one. We evaluate our framework by using it to re-implement an invariance-based rootkit detection system and show the performance benefits of a HyperForce-utilizing countermeasure.

==> Makefile <==

TEXFILES = abstract.tex background.tex conclusion.tex design.tex \
           evaluation.tex hyperforce.tex intro.tex related.tex

all: hyperforce.pdf
	evince hyperforce.pdf &

hyperforce.pdf: ${TEXFILES} hyperforce.bib
	pdflatex hyperforce.tex
	if grep -q "\cite{" *.tex; then bibtex hyperforce; fi
	pdflatex hyperforce.tex
	if grep -q "\cite{" *.tex; then bibtex hyperforce \
         | grep "Warning"; true; fi
	pdflatex hyperforce.tex \
         | egrep "Citation|Reference|Float|Label|Warning";
	

spell: ${TEXFILES}
	for i in ${TEXFILES}; do aspell --lang=en_US --personal=./hyperforce.dict check $$i; done

clean:
	rm -f *.out hyperforce.pdf *.aux *.log *.toc *.lof *.lot *~ *.bak *.cb *.cb2 *.bbl *.blg
	rm -f */*.out */*.aux */*.log */*.toc */*.lof */*.lot */*~ */*.bak


